Plumeria at SemEval-2022 Task 6: Robust Approaches for Sarcasm Detection for English and Arabic Using Transformers and Data Augmentation

This paper describes our submission to SemEval-2022 Task 6 on sarcasm detection and its five subtasks for English and Arabic. Sarcasm conveys a meaning which contradicts the literal meaning, and it is mainly found on social networks. It has a significant role in understanding the intention of the user. For detecting sarcasm, we used deep learning techniques based on transformers due to its success in the field of Natural Language Processing (NLP) without the need for feature engineering. The datasets were taken from tweets. We created new datasets by augmenting with external data or by using word embeddings and repetition of instances. Experiments were done on the datasets with different types of preprocessing because it is crucial in this task. The rank of our team was consistent across four subtasks (fourth rank in three subtasks and sixth rank in one subtask); whereas other teams might be in the top ranks for some subtasks but rank drastically less in other subtasks. This implies the robustness and stability of the models and the techniques we used.

==> related.tex <==
% \section{Related Work}

% Most previous textual sarcasm detection dataset shave been annotated using a weak supervision method. In this approach, texts are  considered sarcastic if they meet predefined criteria, such as including specific tags (e.g. \#sarcasm, \#irony) \cite{ptacek-etal-2014-sarcasm}; \cite{khodak-etal-2018-large}. However, this can lead to noisy labels for several reasons, as outlined by \cite{oprea2020effect} Oprea et. al (2020). Other work has relied on manual labelling, where sarcasm labels are provided by human annotators \cite{filatova-2012-irony}; \cite{riloff-etal-2013-sarcasm}; \cite{abercrombie-hovy-2016-putting}. However, such labels represent annotator perception, which may differ from author intention, as further pointed out by \cite{oprea-magdy-2020-isarcasm}.

% Further, the vast majority of sarcasm detection work \cite{campbell2012there}; \cite{riloff-etal-2013-sarcasm}; \cite{joshi-etal-2016-word}; \cite{zhang-wallace-2017-sensitivity}; \cite{rajadesingan2015sarcasm}; \cite{bamman2015contextualized}; \cite{amir-etal-2016-modelling}; \cite{hazarika-etal-2018-cascade}; \cite{oprea-magdy-2020-isarcasm} has focused exclusively on the English language and, due to the sociocultural aspects of sarcastic communication \cite{oprea-magdy-2020-isarcasm}, it is unclear if models trained on English could generalise to other languages. To our knowledge, the small amount of work on other languages such as Arabic \cite{karoui-etal-2017-exploring}; \cite{ghanem2019idat}; \cite{abbes-etal-2020-daict}; \cite{abu-farha-magdy-2020-arabic} relies on the two labelling methods above.

\subsection{Previous Shared Tasks}

Previous shared tasks on sarcasm detection \cite{VanHee2018}; \cite{ghanem2019idat}; \cite{ghosh-etal-2020-report}; \cite{abu-farha-etal-2021-overview} have only two subtasks; one is sarcasm detection and another is to predict the type of sarcasm. 

% \cite{VanHee2018};
In shared task \cite{VanHee2018}, the systems submitted for both subtasks represent a variety of neural-network-based approaches (i.e., CNNs, RNNs, and (bi-)LSTMs) exploiting word and character embeddings and handcrafted features. Some participants also included other popular classification algorithms: Support Vector Machines, Maximum Entropy, Random Forest, and Naive Bayes. 

% \cite{ghanem2019idat};
In shared task \cite{ghanem2019idat}, the methods of participants submitted mostly similar to \cite{VanHee2018}, ranged from feature-based to neural networks using either classical machine learning techniques or ensemble methods. Some participants also used Transformer based models.


% \cite{ghanem2019idat}; 
Arabic sarcasm detection

This shared task \cite{ghanem2019idat} for Arabic sarcasm detection, in that task, most of the teams used pre-trained language models such as AraBERT \cite{antoun-etal-2020-arabert}, and MARBERT \cite{abdul-mageed-etal-2021-arbert}. A few of the participants used deep learning and conventional machine learning approaches. Additionally, participants utilized a language model to augment the data with new sarcastic examples. The augmentation was done by replacing and adding new words. Some participants used BERT models in different ways. The majority of the participants used ensemble methods, combining BERT-based models with other models. While most participants used the same architecture for both tasks, some participants relied on multi-task learning to train the model on both tasks simultaneously


% \cite{ghosh-etal-2020-report}; 
In shared task \cite{ghosh-etal-2020-report}, almost every submitted system have used transformer-based architectures, such as
BERT \cite{} and RoBERTa \cite{}, and other variants, emphasize the increasing popularity of using pre-trained language models for various classification tasks. However, the best systems have employed a clever mix of ensemble techniques and data augmentation setups.
